Designing Trustworthy Layered Attestations

Attestation means providing evidence that a remote target system is worthy of trust for some sensitive interaction. Although attestation is already used in network access control, security management, and trusted execution environments, it mainly concerns only a few system components. A clever adversary might manipulate these shallow attestations to mislead the relying party. Reliable attestations require layering. We construct attestations whose layers report evidence about successive components of the target system. Reliability also requires structuring the target system so only a limited set of components matters. We show how to structure an example system for reliable attestations despite a well-defined, relatively strong adversary. It is based on widely available hardware, such as Trusted Platform Modules, and software, such as Linux with SELinux. We isolate our principles in a few maxims that guide system development. We provide a cogent analysis of our mechanisms against our adversary model, as well as an empirical appraisal of the resulting system. We also identify two improvements to the mechanisms so attestation can succeed against strengthened adversaries. The performance burden of our attestation is negligible, circa 1.3 percent. After our first example, we vary our application level, and then also its underlying hardware anchor to use confidential computing with AMD's SEV-SNP. The same maxims help us achieve trustworthy attestations.

==> am_exclusive_access_to_its_key.tex <==
Why does the attestation signing key \ask{} speak for the Attestation
Manager reliably, by means of the \texttt{tpm\_sign} executable?  That
is, why should we believe that whenever we observe a message $m$
signed with \ask{}, then the Attestation Manager requested that $m$ be
signed?

\paragraph{Preferred strategy.}  A good answer to this question \emph{could}
take the following form, if the right underlying mechanisms were
available.  This involves IMA, the SELinux policy, and the TPM
locality mechanism working together.
%
\begin{enumerate}
  \item \ask{} is wrapped with a key
  policy stipulating that each signing command require a
  configuration-compliant PCR state $P_A$, and that the command should
  be delivered to the TPM labeled with a particular locality $A$.
  \item The kernel, when running our SELinux policy, labels commands
  with locality $A$ only when the request is delivered by a process
  running in domain $D_A$.\label{item:lkernel:locality:label}
  \item Our SELinux policy assigns domain $D_A$ only to the executable
  at a particular path in the filesystem, \texttt{tpm\_sign} in our
  case, which can be invoked only from a domain $D_{AM}$ that only AM
  instances run within.
  \item Our IMA policy enforces that the \texttt{tpm\_sign} and AM
  executables have the hashes determined for the correct signing
  program and Attestation Manager.
  \item The PCR state $P_A$ incorporates our SELinux and IMA policies.  
\end{enumerate}
%
The problem with using this rather direct strategy is that standard
kernels have no code to deliver commands with TPM localities, and
associating TPM localities with specific application-level processes
is also unsupported, even via SELinux.  Thus,
item~(\ref{item:lkernel:locality:label}) is not currently
implementable.  The only reliably delivered localities are generated
by the underlying hardware for some early-boot, hardware-generated
events.

One of our key recommendations is for the maintainers of
Linux and SELinux to make the necessary changes to enable use of the
versatile TPM locality mechanism.

\paragraph{A practical strategy.}  A stopgap solution diverges from
Maxim~\ref{maxim:resist:transitory:corruption} on resilience against
transient corruptions, but provides some protection against misuse of
\ask{}.  The stopgap approach omits the locality
requirement from the key policy, specifying only the required TPM PCR
values.  This approach maintains the wrapped \ask{} with its
policy as a secret, stored in a double-wrapped form.  The key pair
used in the external wrapping constrains decryption
events to the pre-release PCR state. 
\ask{} can be used only if the PCRs are in the post-release state,
reflecting a proper boot with IMA and SELinux running with our
intended policies.
\texttt{pol\_scr} unwraps the external layer to place the single-wrapped
key blob in the filesystem so that only \texttt{tpm\_sign} can read
it, and then extends the PCRs to the post-release state.
Thus, the single-wrapped key blob will be accessible only to
\texttt{tpm\_sign}, and only when the boot has successfully installed
our SELinux and IMA protections.  When \texttt{tpm\_sign} delivers the
key blob in a TPM authenticated session, each signing command
authenticates itself as the source of the command.  When the session
concludes, the TPM flushes the key blob.

The stopgap reduces the divergence from
Maxim~\ref{maxim:resist:transitory:corruption}, as an adversary that
causes the computer to execute a different boot process does not
obtain the single-wrapped key blob.  By contrast, a fast and
determined adversary exploiting a kernel weakness can obtain the
single-wrapped key blob from the SELinux-protected file.  It must then
heal any damage to the kernel so LKIM does not disclose the intrusion.
It can subsequently impersonate the AM to obtain signatures whenever
desired.  Although this approach does not resist \emph{very}
transitory corruptions, it resists boot-cycle length corruptions.

As a fine point, our demo uses a variant.  Delivering the key blob
each time takes a long time on actual TPMs.  Moreover, generating new
keys each time the target PCRs would vary was unmanageable during our
development.  Instead, we used a \emph{delegated key usage policy},
also known as a ``wildcard
policy''~\cite{Arthur:2015:A-Practical-Guide-to-TPM-2.0-Certifying-Keys}.
This delegates authority to a policy signer by including a fingerprint
of their verification key when generating a new TPM-resident key.  The
signer provides the actual key policies by signing them with that verification key.
However, an appraiser receiving signed evidence does not know which
{delegated key usage policy} was presented to yield this particular
signature, weakening adherence to
Maxim~\ref{maxim:display:boot:trait}.

% This stopgap solution benefits from the fact that the AM is already
% an exception to Maxim~\ref{maxim:short:lived}, namely rather than
% being a short-lived process, it is started in the boot process and
% persists though the platform runtime.

Other strategies could also provide ways to associate the \ask{}
exclusively with the actions of the AM.  For instance, Trusted
Execution Environments, TEEs such as SGX, TDX, SEV, as well as
research proposals such as Sancum and
CAIF~\cite{cryptoeprint:2016:086,cheng2023intel,misono2024confidential,Noorman:SancusL2017,GuttmanEtAl2025},
may allow unambiguous evidence of the process delivering commands
through a channel.  In our work, we kept our focus on more generic
hardware.
  


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "cds-demo25"
%%% End:

